Searching for Molecular Signatures in 14 Transiting Exoplanets with SPIRou

High-resolution spectroscopy provides unique constraints on exoplanet atmospheric composition and dynamics. The past decade of ground-based campaigns has accumulated extensive public archives, yet many observations remain unanalysed. We present a homogeneous blind-search analysis of 50 SPIRou transits spanning 14 exoplanets, ranging from super-Earths to ultra-hot Jupiters, combining data from large program and public archived observations. Using automated data reduction and atmospheric retrieval via Nested Sampling validated by Cross Correlation Function analysis, we confirm previous H2O and CO detections in HD 189733 b, WASP-76 b, and WASP-127 b, report tentative H2S detections in HD 189733 b and TOI-1807 b, tentative detection of GJ 3470 b's atmosphere, and provide upper limits for non-detections. This work demonstrates a scalable method for systematic archive analysis, providing a first step toward ground-based support of large space-based atmospheric characterization programs and the study of atmospheric diversity across exoplanet populations from a statistical perspective.

==> macros.tex <==
% macros.tex
% Custom LaTeX macros for exoplanet/SPIRou papers

% Ensure xspace is available when this file is loaded in the preamble
\RequirePackage{xspace}

% Units
\newcommand{\kms}{\,km\,s$^{-1}$\xspace}
\newcommand{\ms}{\,m\,s$^{-1}$\xspace}
\newcommand{\mum}{\,$\mu$m\xspace}
\newcommand{\Rsun}{\,R$_\odot$\xspace}
\newcommand{\Msun}{\,M$_\odot$\xspace}
\newcommand{\Rjup}{\,R$_\mathrm{Jup}$\xspace}
\newcommand{\Mjup}{\,M$_\mathrm{Jup}$\xspace}
\newcommand{\Rearth}{\,R$_\oplus$\xspace}
\newcommand{\Mearth}{\,M$_\oplus$\xspace}
\newcommand{\Teff}{T$_\mathrm{eff}$\xspace}
\newcommand{\logg}{\log g\xspace}
\newcommand{\FeH}{[Fe/H]\xspace}
\newcommand{\vsini}{$v\sin i$\xspace}
\newcommand{\snr}{S/N\xspace}
\newcommand{\chisq}{$\chi^2$\xspace}
\newcommand{\chisqdof}{$\chi^2_\nu$\xspace}
\newcommand{\angstrom}{\,\text{\normalfont\AA}\xspace}
\newcommand{\BJD}{BJD$_\mathrm{{TDB}}$}

% Planets & stars
\newcommand{\mjup}{\,M$_{\rm Jup}$\xspace}
\newcommand{\rjup}{\,R$_{\rm Jup}$\xspace}
\newcommand{\mearth}{\,M$_{\oplus}$\xspace}
\newcommand{\rearth}{\,R$_{\oplus}$\xspace}
\newcommand{\msun}{\,M$_{\odot}$\xspace}
\newcommand{\rsun}{\,R$_{\odot}$\xspace}

% Astronomy
\newcommand{\Lsun}{\,L$_\odot$\xspace}
\newcommand{\Lstar}{\,L$_\star$\xspace}
\newcommand{\Mstar}{\,M$_\star$\xspace}
\newcommand{\Rstar}{\,R$_\star$\xspace}
\newcommand{\Mplanet}{\,M$_\mathrm{p}$\xspace}
\newcommand{\Rplanet}{\,R$_\mathrm{p}$\xspace}

% Abbreviations
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\etc}{etc.\xspace}
\newcommand{\cf}{cf.\xspace}
\newcommand{\vs}{vs.\xspace}
\newcommand{\degree}{\,$^\circ$\xspace}
\newcommand{\logt}[1]{\mathrm{log}_{10}(#1)\xspace}

% Math
\newcommand{\dd}{\mathrm{d}}
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\deriv}[2]{\frac{\dd #1}{\dd #2}}

% Atmo
\newcommand{\Tiso}{$\mathrm{T}_\mathrm{iso}$\xspace}
\newcommand{\Vrot}{$\mathrm{V}_\mathrm{rot}$\xspace}


% Misc
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\fixme}[1]{\textcolor{orange}{FIXME: #1}}
% \newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\red}[1]{{#1}}

% Add more macros as needed!
